Average-Case Hardness of Parity Problems: Orthogonal Vectors, k-SUM and More

This work establishes conditional lower bounds for average-case {\em parity}-counting versions of the problems $k$-XOR, $k$-SUM, and $k$-OV. The main contribution is a set of self-reductions for the problems, providing the first specific distributions, for which: $\mathsf{parity}\text{-}k\text{-}OV$ is $n^{\Omega(\sqrt{k})}$ average-case hard, under the $k$-OV hypothesis (and hence under SETH), $\mathsf{parity}\text{-}k\text{-}SUM$ is $n^{\Omega(\sqrt{k})}$ average-case hard, under the $k$-SUM hypothesis, and $\mathsf{parity}\text{-}k\text{-}XOR$ is $n^{\Omega(\sqrt{k})}$ average-case hard, under the $k$-XOR hypothesis. Under the very believable hypothesis that at least one of the $k$-OV, $k$-SUM, $k$-XOR or $k$-Clique hypotheses is true, we show that parity-$k$-XOR, parity-$k$-SUM, and parity-$k$-OV all require at least $n^{\Omega(k^{1/3})}$ (and sometimes even more) time on average (for specific distributions). To achieve these results, we present a novel and improved framework for worst-case to average-case fine-grained reductions, building on the work of Dalirooyfard, Lincoln, and Vassilevska Williams, FOCS 2020.

==> NotesForIntro.tex <==

Emphasis points:
\begin{itemize}
    \item Cool Results
        \begin{itemize}
            \item First (we think) average-case parity SAT hardness. 
            \item First (confident) average-case parity hardness for $k$-OV, $k$-XOR, $k$-SUM.
            \item First tight hardness in the average-case for counting or parity SAT. : 1989-1991 improvement over
        \end{itemize}
    \item Cool techniques \mina{we have a techniques section that these mostly go there.} \andrea{++}
        \begin{itemize}
            \item To get our hardness for $\paritySAT$, $\paritykSUM$, $\paritykOV$, and parity $k$-XOR we show worst-case to worst-case reductions from factored problems to normal (not factored) problems.  In \cite{factoredProblems} they show hardness for $k$-LCS from factored problems, however, $k$-LCS is much more expressive than $k$-OV. As evidence of $k$-LCS's expressiveness, it branching programs can be reduced to LCS (where as for $k$-OV we only know how to do it from SAT) \cite{AbboudHWW16}. In this paper we truly go from the $k$-OV hypothesis to average-case $\paritykOV$ closing the loop of the previous reduction \cite{factoredProblems}. We close the loop on the other problems studied in \cite{factoredProblems} $k$-SUM and $k$-XOR. We also demonstrate hardness for SAT.
            \item We improve the framework of \cite{factoredProblems}, these improvements allow us to show hardness for computing parity (as opposed to counting over the integers). Additionally, these improvements result in faster reductions, improving the overhead from $\lg(n)^{d}$ to $2^d$. We answer several open problems from \cite{factoredProblems}. 
                \begin{itemize}
                    \item \textit{Can the framework be improved? For example, could it be improved to handle polynomials of (slightly) greater degree? Can the strong k-partiteness condition be weakened? }
                    \item \textit{What other natural non-factored problems are hard from factored problems?}
                \end{itemize}
        \end{itemize}
    \item 
\end{itemize}






\barna{Question 1. What are the major improvements over DLW20? PLease elaborate. What are the theorem statements (just give reference) that shows those improvements.}

Please elaborate on the following:
\begin{itemize}
    \item {\bf Why} improvement in the framework of DLW20 is important? State that DLW20 framework was an improvement over Boix-Adsera et al. 2019, and what new things you could achieve due to that in DLW20 over Boix-Adsera et al. 2019, and what remained open.
    \item State {\bf how} you improved over the framework of DLW20 (you mentioned that it already handled parity--so that is not a new thing.) \andrea{DLW didn't handle parity. BBB19 could do parity for cliques, but, we didn't take their result and make it work in the framework. }
    
\end{itemize}

In this paper we have two major improvements over the results from \cite{factoredProblems}. The first is that we get worst-case to average-case self-reductions for partiy counting versions of SAT, $k$-OV, $k$-SUM, and $k$-XOR. In \cite{factoredProblems} they show that counting \emph{factored} versions of these problems are hard on average. In this paper we show average-case hardness for parity counting SAT, $k$-OV, $k$-SUM, and $k$-XOR and not an altered version of these problems. 

We also improve the framework itself. Our new framework is more efficient. Given a $d$ degree polynomial we have an overhead of $2^d$ instead of $\lg(n)^d$. This improvement makes the reductions stronger. Additionally, the \cite{factoredProblems} framework only works for counting problems over large fields (as stated in their papers they talk about this over the integers in fact). In this paper we improve this framework to work for parity. Furthermore, we remove a condition on the polynomials that work in this framework. In \cite{factoredProblems} there is a restriction that the polynomial must be `strongly k-partite'. This is a restriction on the structure of the monomials that are allowed in polynomials. In this paper we remove this restriction, and thus only have the restriction that the polynomial be sufficiently low-degree. 


\barna{Question 2. What was the state of the art for parity SAT, and counting SAT? How we progress on that? What are the theorems showing that?}

To the best of my knowledge there was no known average-case distribution on which parity SAT was known to be hard. So we present (to my knowledge) the first result of this type. 
For counting SAT there was a lower bound from the permanent. I believe the permanent was shown to be hard in \cite{Lipton89} and \cite{FeigenbaumF91}. \andrea{@Vinod and @Virginia, do you know if there is anything else we should cite?} \vnote{The paragraph I wrote in the related work section has the relevant citations.} From the permanent they get a average-case distribution on which SAT has a lower bound of $2^{\Omega(\sqrt{n})}$. This is far from tight, we however find an average-case distribution on which SAT is $2^{\Omega(n)}$ hard. 

\barna{Question 3. What is the current state of art on parity problems? Are there evidence that decision problems are almost always as hard as parity problems? Are there evidence that parity problems are easier than their counting versions? Give the references.}

For all of the problems we consider here there isn't a substantial speed up in the worst-case between decision, parity and counting versions of problems. In reductions land have reductions that show that $decision<parity<counting$ unsurprisingly. I don't know of any reductions that demonstrate a `surprising' direction of reduction for the problems we are studying. So, I know of no reduction from parity to decision for any of the problems we discuss here. I also know of no reduction from counting to parity for any of the problems we discuss here. 

There has been a study of parity hardness in FGC \cite{AbboudParity}. In their paper they show that parity and decision are equivalent for many problems, like APSP. However, they also show that the parity counting version of is, conditionally, strictly harder for negative weight triangle than the decision version of negative weight triangle. In \cite{AbboudParity} they don't get results for parity vs decision for the problems we consider in this paper. 
%I will note that if an explicit reduction existed from parity to decision for our problems we could build a fine-grained one-way function from the associated worst-case hypotheses. \vnote{This isn't clear to me: one-way functions need an easy direction, in addition to a hard direction. Typically, the easy direction is to sample a hard problem (from a distribution) {\em together with its solution}. Assuming there is a reduction from a parity problem to the decision problem, where do you get the easy direction from?} 
%This is a still open problem stated in  \cite{BallWorstToAvg}. So, while we don't have such a reduction this paper does create an exciting implication of such a reduction. 

\andrea{================}

==> OldFiles/DenseOV.tex <==
\subsection{How Hard is Dense Counting k-OV in the Uniform Average Case?}
\xxx{Issue with this section: $2^d$ is too expensive. It would be fine if we could say no alg works for $2^{o(d)}$. }

First, let us clarify what we mean by the dense $\#k$-OV problem. We are simply referring to the fact that if the vectors are of length $d$ we expect instances to have approximately $n=2^d/2$ vectors. At a high level what we are going to do is take Lemma \ref{lem:dimensionReduction} and hide our $k$-partite instance in series of dense random instances of the $\#k$-OV problem.
We will now give a definition of the random dense $k$-OV distribution. 

\newcommand{\DdDkOV}{D_{d,DkOV}}
\begin{definition}
Let $D_{d,S}$ be the uniform distribution over sets of vectors of length $d$. Specifically, over all $2^{2^d}$ possible sets of strings of length $d$  we draw each individual string with probability  $2^{-2^d}$. 

Let $\DdDkOV$ be the distribution over $k$ sets of vectors, $S_1,\ldots,S_k$ where all vectors have dimension $d$. To sample an instance from $\DdDkOV$ simply draw each set $S_i$ iid from $D_{d,S}$.
\end{definition}

\begin{lemma}
An algorithm $\alg$ which succeeds with probability $1-2^{-k}/3$ on instances of $\oplus k$-OV drawn from $\DdDkOV$ in time $T(d)$ implies a randomized algorithm exists for worst case instances of $\oplus k$-OV on vectors of length $d$ that runs in time $O\left( 2^k(T(d) +2^d) \right)$ which succeeds with probability $2/3$.
\label{lem:denseOVWCtAC}
\end{lemma}
\begin{proof}
Given a $k$-partite worst case instance, $I_0$, of $k$-OV with vectors of length $d$ in lists $L_1,\ldots, L_k$
create vectors $\ell_1,\ldots,\ell_k$ of length $2^d$ for each of the $k$ partitions where 
$$\ell_i[v] =\begin{cases}
1& \text{ if } v\in L_i \\
0& \text{ if } v \notin L_i\end{cases}.$$
Now draw a random instance $I_R \sim D_{d,DkOV}$ which has lists $R_1,\ldots, R_k$. As before create vectors $r_1,\ldots,r_k$ of length $2^d$ for each of the $k$ partitions where 
$$r_i[v] =\begin{cases}
1& \text{ if } v\in R_i \\
0& \text{ if } v \notin R_i\end{cases}.$$
Let 
$$c_i^j =\begin{cases}
r_i& \text{ if }j=0 \\
r_i \oplus t_i & \text{ if }j=1 \end{cases}.$$
Let $C_i^j = \{v | c_i^j[v] =1\}.$
We will now create $2^k$ instances of $k$-OV. These instances correspond to inputs with lists $C_1^{j_1},\ldots,C_k^{j_k}$ for all possible choices of $j_i \in \{0,1\}$. 
We then use  inclusion exclusion to get the count of $I_0$ from these various instances.  We will now argue two points. First, that these instances look random. Second, that after $2^k$ correctly answered calls we will solve the worst case problem.

We want to argue that for any fixed choice of $j_1,\ldots,j_k$ the instance $C_1^{j_1},\ldots,C_k^{j_k}$ is drawn from $D_{d,DkOV}$. Obviously, between different choices of  $j_1,\ldots,j_k$  the instance look correlated, however, we will use union bound over these correlated instances to argue that our success probability is high enough. First note that for any $j_i=0$ the set $C_i^{j_i}=C_i^0$ is drawn from  $D_{d,S}$ by definition. For any $j_i=1$ first note that the bit-wise XOR of any vector and a uniformly random $\{0,1\}$ vector is itself a uniformly random vector. Given this $C_i^{j_i}=C_i^1$ is drawn from  $D_{d,S}$ as well. So, for any fixed $j_1,\ldots,j_k$ we have that $C_1^{j_1},\ldots,C_k^{j_k}$ is drawn from $D_{d,DkOV}$.

First note that we will get correct answers on all of our $2^k$ instances with probability at least $2/3$ by union bound.
If we have correct answers for all of our $2^k$ calls then we can XOR all of the answers to the calls to get the answer for our original problem $I_0$. Let $T$ be the set of all $k$ tuples of $d$ length vectors $(v_1,\ldots,v_k)$ which form an orthogonal $k$-tuple. Now note that the $\oplus k$-OV of $I_0$ is 
$$\bigoplus_{(v_1,\ldots,v_k) \in T} \ell_1[v_1]\cdot \ell_2[v_2] \cdots \ell_k[v_k] .$$
Similarly, the $\oplus k$-OV of $ C_1^{j_1},\ldots,C^{j_k}_k$ is 
$$\bigoplus_{(v_1,\ldots,v_k) \in T} c^{j_1}_1[v_1]\cdot c^{j_2}_2[v_2] \cdots c^{j_k}_k[v_k] .$$
Finally, note that for each of these monomials 
$$\bigoplus_{j_1,\ldots,j_k \in \{0,1\}} c^{j_1}_1[v_1]\cdot c^{j_2}_2[v_2] \cdots c^{j_k}_k[v_k]  = \ell_1[v_1]\cdot \ell_2[v_2] \cdots \ell_k[v_k].$$
This means that the XORs of all of our answers to the $2^k$ instances result in $\bigoplus_{(v_1,\ldots,v_k) \in T} \ell_1[v_1]\cdot \ell_2[v_2] \cdots \ell_k[v_k]$, which is in fact the answer to instance $I_0$.

An algorithm $\alg$ which succeeds with probability $1-2^{-k}/3$ on instances of $\oplus k$-OV drawn from $D_{d,DkOV}$ in time $T(d)$ implies a randomized algorithm exists for worst case instances of $\oplus k$-OV on vectors of length $d$ that runs in time $O\left( 2^k(T(d) +k2^d) \right)$ which succeeds with probability $2/3$. The overhead of $2^{k+d}$ in our running time comes from generating the inputs to all of the instances. 

\end{proof}

Now that we have this reduction, what does it imply for the hardness of these dense instances? 

\begin{theorem}
We restrict $k$ to $k = o(\lg(n))$.
There exists a constant $c$ such that $\oplus k$-OV instances drawn from $\DdDkOV$ when $d= ck\lg(n)$ require $n^{\Theta(k)}$ time if SETH is true. \xxx{Also from ETH but we need that lemma statement.}
\end{theorem}
\begin{proof}
By Lemma \ref{lem:dimensionReductionETH} there exists a constant $c$ such that $k$-OV problem on $N$ vectors of length $kc\lg(N)$ requires $N^{\Theta(k)}$ time. By Lemma \ref{lem:decisionToParity} this gives the same hardness for the $\oplus k$-OV problem. 
 
Assume for the sake of contradiction that an algorithm exists for $\oplus k$-OV instances drawn from $\DdDkOV$ when $d= c\lg(N)$ (note that the number of vectors is at most $n=kN^{c}$) have an algorithm which runs in time $n^{o(k)}$ with probability $1-2^{-k}/3$. Note that we can phrase this running time in terms of $d$ as $2^{d o(k)}$.
Now we will use Lemma \ref{lem:denseOVWCtAC} to note that this implies a randomized algorithm for worst case $k$-OV on $c\lg(N)$ length vectors which runs in time $O( 2^k N^{c o(k)} 2^{c \lg(N)})$. Now we state this as an exponential with a base of $n$ $O(n^{k/lg(N) + co(k) + c})$. Now note that $k/lg(n) + co(k) + c = o(k)$. This is a contradiction, as it offers a faster algorithm than $N^{\Theta(k)}$ for worst case $k$-OV! 
\end{proof}

==> OldFiles/KcubedOldresult.tex <==
\subsection{Previous Work}
Next we will recall the results of three Lemmas from \cite{factoredProblems} which together show that $\oplus$\ckxor, $\oplus$\ckov, and $\oplus$\cksum~can be reduced to each other. 

\begin{theorem}[\cite{factoredProblems} (Lemma 3.3, Lemma 3.4 and Theorem 1.7)]
\label{thm:completenessOfFactoredProblems}
If we can solve  \#\ckxor[], \#\ckov, or \#\cksum with $g$ sets of $k^3b$ length vectors in time $T(n)$ then we can solve \#\ckfunc[]~instance with $g$ sets of $b$ length vectors in time $T(n)+\tilde{O}(n)$. 

Additionally, 
Let $v_1, \ldots, v_k$ be $k$ factored vectors each with $g$ subsets of $\{0,1\}^b$. Let $f_{XOR}$ be the function that returns $1$ if the $k$ input vectors XOR to zero and otherwise returns $0$. 
There is a function $\gamma_{\mathfrak{f} \rightarrow XOR,k}(\cdot, \cdot)$ that takes as input a factored vector with $g$ subsets of $\{0,1\}^b$ and an index and returns a new factored vector  with $g$ subsets of $\{0,1\}^{O(b)}$. This function $\gamma_{\mathfrak{f} \rightarrow XOR,k}$ 
runs in $\tO(2^b \cdot g)$ time for each vector and:
$$\circledcirc_{f_{XOR}}(\gamma_{\mathfrak{f} \rightarrow XOR,k}(v_1, 1), \ldots, \gamma_{\mathfrak{f} \rightarrow XOR,k}(v_k,k)) = \circledcirc_{\mathfrak{f}}(v_1, \ldots, v_k).$$
\end{theorem}

In fact the counts are exactly the same. So, it is also the case that $\oplus$\ckxor[]~with $g$ sets of $k^3b$ length vectors in time $T(n)$ then we can solve $\oplus$\ckfunc[] with $g$ sets of $b$ length strings in time $T(n)$. The reductions between each of these functions to the other blow up the size of $bg$ by a factor of $k^3$.

So this previous work implies the existence of:
\begin{itemize}
    \item $\oplus (f,n,k,b,g) \rightarrow (OV, n,k,bk^3,g)$,
    \item $\oplus (f,n,k,b,g) \rightarrow (SUM, n,k,bk^3,g)$,
    \item and $\oplus (f,n,k,b,g) \rightarrow (XOR, n,k,bk^3,g)$
\end{itemize}
reductions. 


==> OldFiles/ac-ov-sum-xor-hard.tex <==
\subsection{How hard is Counting k-OV on Average?}
\label{subsec:smallDimOVhard}


We will start by giving hardness for $\oplus$\ckov~in the average-case using our previous lemmas and theorems. Then we will give a reduction from $\oplus$\ckov~to $k'$-OV. Depending on the hypotheses we start with we will have different values of implied hardness. 

\begin{lemma}
Let $P_{b,g}$ be the problem of solving $\oplus$\ckov$(n,b,g)$~drawn from the uniform average-case distribution with $g$ sets of vectors of length $b$ with probability $ 1-\frac{2^{-kg}}{8}$, where $kg = o(\lg(n)/\lg\lg(n))$ and $bg=O(k\lg(n))$.%\mina{I added this since Lemma \ref{lem:selfReductionsWithbg} requires it }%Additionally we restrict $kg = o(\lg(n)/\lg\lg(n))$ for the rest of this lemma.  
\xxx{Andrea: is the gamma thing O() or not?}
\begin{itemize}
\item %Assuming the $k$-XOR hypothesis, if an $\oplus (XOR,n,k,b,g) \rightarrow \oplus(OV, n,k,O(\frac{gb^2}{k\lg(n)}),g)$ reduction exists which takes $n^{o(k)}$ time then
Assuming the $k$-XOR hypothesis, if an $\oplus $\ckxor$(n,b,g) \rightarrow \oplus $\ckov[]$(n,O(\frac{gb^2}{k\lg(n)}),g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{b,g}$ requires $n^{\lceil k/2 \rceil-o(1)}2^{-kg}$ time. %if $gb = \gamma(k)k\lg(n)$.
\item Assuming the $k$-SUM hypothesis, if an %$\oplus (SUM,n,k,b,g) \rightarrow (OV, n,k,O(\frac{gb^2}{k\lg(n)}),g)$
$\oplus $\cksum[]$(n,b,g) \rightarrow \oplus $\ckov$(n,O(\frac{gb^2}{k\lg(n)}),g)$
reduction exists which takes $n^{o(k)}$ time then $P_{b,g}$ requires $n^{\lceil k/2 \rceil-o(1)}2^{-kg}$ time. %if $gb = \gamma(k)k\lg(n)$.
\item 
Assuming SETH, for every constant $\epsilon>0$ $P_{b,g}$ requires $n^{k (1-\epsilon)-o(1)}2^{-kg}$ time for $g,b$ where $gb = kc_\epsilon \lg(n)$ for some fixed constant $c_\epsilon$. %\mina{is it for every $\epsilon$? since we have $bg=O(k\lg(n))$, is the if statement necessary?}
\item Assuming ETH,  $P_{b,g}$ requires $n^{\Omega(k)}2^{-kg}$ time as long as $bg>ck\lg(n)$ for some large global constant $c$ (this constant comes from ETH). \mina{I guess the if statement is not necessary here since it is capture above and there is no epsilon.} \xxx{Note: how can we make this clear? The $c$ depends on what the constants from ETH and sparisfication are, so the user of the lemma can't pick them. How do we make that clear.}
\end{itemize}

\label{lem:FOVfromNormalVerisons}
\end{lemma}
\begin{proof}
For the first two statements we will use Lemma 
\ref{lem:selfReductionsWithbg}. Then we use the definition of the reduction from Definition \ref{def:bgReduction}. Then apply Theorem \ref{thm:frameworkImprovement}. 

The second to last statement is the same as the statement from Lemma 
\ref{lem:selfReductionsWithbg}. Then apply Theorem \ref{thm:frameworkImprovement}.

The last statement uses Lemma\ref{lem:selfReductionsWithbg} with Theorem \ref{thm:frameworkImprovement}.
\end{proof}

We will give an explicit distribution from which we are drawing our average-case instances of $k$-OV.

\begin{definition}\mina{why is this showing as definition 1? definition 1 is something else and there is no error in labeling that I can see.} \xxx{TODO: fix definition in commands of defintion st this doesn't happen.}
We define the distribution $D_{OV}(k,n,b,g)$ to be a distribution over inputs to $gk$-OV. This input is generated by taking uniformly random instances of $\oplus$\ckov~with $k$ lists of $n$ factored vectors where each factored vector is made up of $g$ sets of $b$ length vectors and then applying the reduction from Theorem \ref{thm:factoredToUnfactored}.
Note that input sizes of instances drawn from $D_{OV}(k,n,b,g)$ are $N= n 2^b g k$. 
\end{definition}

Now we are going to use our reductions from factored to non-factored problems, plus the hardness of factored problems to get lower bounds for average-case non-factored problems. Note that we are choosing $b=\lg(n)$ because it optimizes the resulting lower bounds and reduction overheads. We are still framing the hardness of these problems in terms of the hardness of the \emph{origional} problem sizes. 

\mina{Since $q$ is the same value all the time, I removed it as a parameter to keep things simple} 
\begin{lemma}
Let $P_{K,N,b,g}$ be the problem of solving $\oplus K$-OV~drawn from $D_{OV}(k,n,b,g)$,  where $N= n 2^b g k$ and $K=gk=o(\lg(n)/\lg\lg(n))$ with probability $q = 1-\frac{2^{-k}}{8}$. %Additionally we restrict $K=kg = o(\lg(n)/\lg\lg(n))$ for the rest of this lemma. 
\begin{itemize}
    \item Assuming ETH, there exists some $c$ such that for $b=\lg(n)$ and $g=ck$, $P_{K,N,b,g}$ (which can also be writen as  $P_{ck^2,N, \lg(n), ck}$) requires $n^{\Theta(k)}$ time. %\mina{is the $N$ supposed to be capital or small? same question for $k$, since the definitions above make this statement confusing}% if ETH is true. 
    \item Assuming the $k$-SUM hypothesis, if an $\oplus (SUM,N,k,b,g) \rightarrow (OV, n,k,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then setting $b=\lg(n)$ and $g=k\gamma(k)$ we can show that $P_{K,N,b,g}$ (a.k.a $P_{k^2 \gamma(k),N,\lg(n),k\gamma(k)}$) requires $n^{\lceil k/2 \rceil}$ time.\mina{$\gamma(k)$ can be anything or is it $gb/k\lg(n)$ like above? answer: gamma is a variable here} % if the $k$-SUM hypothesis is true.
    \item Assuming the $k$-XOR hypothesis, if an $\oplus (XOR,n,k,b,g) \rightarrow (OV, n,k,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then setting $b=\lg(n)$ and $g=k\gamma(k)$ then $P_{K,N,b,g}$ (a.k.a $P_{k^2 \gamma(k),N,\lg(n),k\gamma(k)}$) requires $n^{\lceil k/2 \rceil}$ time.% if the $k$-XOR hypothesis is true.
\end{itemize}
\label{lem:OVModularLemma}
\end{lemma}
\begin{proof}
For each of these statements we start by using Lemma \ref{lem:FOVfromNormalVerisons} to show hard average case $\oplus$\ckov~is from the relevant hypotheses. Then we apply Theorem  \ref{thm:factoredToUnfactored} to go from the factored version to un-factored. By definition running the uniform distribution of \ckov~through our reduction results in $D_{OV}(k,n,b,g)$. Given the resulting versions we pick $b=\lg(n)$.
\end{proof}



Now we will plug in our actually existing reductions.

\begin{theorem}
Let $P_{q,K,N,b,g}$ be the problem of solving $\oplus K$-OV~drawn from $D_{OV}(k,n,b,g)$. Where $N= n 2^b g k$ and $K=gk$, note that $N$ is the input size to the $\oplus K$-OV problem. Let $q = 1-\frac{2^{-k}}{3}$ for the rest of this lemma. Additionally we restrict $K=kg = o(\lg(n)/\lg\lg(n))$ for the rest of this lemma.

If ETH is true $P_{q,K,N, \lg(n), c}$ requires $N^{\Theta(\sqrt{K})}$ time.

If the $k$-XOR hypothesis is true then $P_{q,k^2 \gamma(k),N,\lg(n),k\gamma(k)}$ requires $N^{ K^{1/3}/4}$ time.

If the $k$-SUM hypothesis is true then $P_{q,k^2 \gamma(k),N,\lg(n),k\gamma(k)}$ requires $N^{ K^{1/3}/4}$ time.

\label{lem:OVonAverage}
\end{theorem}
\begin{proof}
For each of these statements we start by using Lemma \ref{lem:OVModularLemma}. We use the $\gamma = 2k$ that comes from Theorem \ref{thm:ovXORsumFromAny}. Then we convert into $N$ and $K = 2k^2$.

There exists some $c$ such that the $P_{q,K,N, \lg(n), kc}$ problem requires $n^{\Theta(k)}$ time if ETH is true. Note that $K = ck^2$ and $N=n^2$, so the statement can be rewritten as a problem from $P_{q,K,N, \lg(n), c}$ requiring $N^{\Theta(\sqrt{K})}$ time. 

From Lemma \ref{lem:OVModularLemma}, if an $\oplus (SUM,N,k,b,g) \rightarrow (OV, n,k,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then  $P_{q,k^2 \gamma(k),N,\lg(n),k\gamma(k)}$ requires $n^{\lceil k/2 \rceil}$ time if the $k$-SUM hypothesis is true. So plug in $K^{1/3} = k$ and $N^{1/2} =n$. So we get a lower bound of $N^{K^{1/3}/4}$.

An $\oplus (XOR,n,k,b,g) \rightarrow (OV, n,k,kb,g)$ reduction exists which takes $n^{o(k)}$ time so $P_{q,k^2 \gamma(k),N,\lg(n),k^2}$ requires $n^{\lceil k/2 \rceil}$ time if the $k$-XOR hypothesis is true. So plug in $K^{1/3} = k$ and $N^{1/2} =n$. So we get a lower bound of $N^{ K^{1/3}/4}$.
\end{proof}




\begin{lemma}
Assuming SETH there exists fixed constant $c_\epsilon$ such that $\forall c\geq c_{\epsilon}$ the $k$-OV problem with $n$ vectors each of length $ck\lg(n)$ requires $n^{k(1-\epsilon-o(1))}$ time.
\label{lem:dimensionReductionSETH}
\end{lemma}
\begin{proof}
We are going to use the $\ell$-SAT problem, where the number of variables is $n$ and the number of clauses is $m$.
SETH implies that for all constants $\epsilon>0$ there is some $\ell_\epsilon$ such that $\ell_\epsilon$-SAT requires at least $poly(m)2^{n(1-\epsilon-o(1))}$ time. If no such $\ell_\epsilon$ existed for some constant $\epsilon$, then the $\ell$-SAT problem would have an $O(poly(m)2^{n(1-\epsilon+o(1))})$ algorithm for all constant values of $\ell$. This would contradict SETH.

We can now use the Sparsification Lemma from Calabro, Impagliazzo and Paturi \cite{CalabroIP06} to state that if $\ell_{\epsilon/2}$-SAT requires $2^{n(1-{\epsilon/2}-o(1))}$ time then $\ell_{\epsilon/2}$-SAT with at most $m=(2\ell_{\epsilon/2}/\epsilon)^{3\ell_{\epsilon/2}}n$ clauses requires $2^{n(1-\epsilon-o(1))}$ time. 

Now we can use the standard reduction from sparsified $\ell_{\epsilon/2}$-SAT to $k$-OV \cite{ryanThesis}. In this reduction we create $N = 2^{n/k}$ vectors of length $d=m=(2\ell_{\epsilon/2}/\epsilon)^{3\ell_{\epsilon/2}}n$. 
We split the variables into $k$ groups of $n/k$ vectors. Each vector represents a way to set $n/k$ variables, location $i$ of the vector is a zero if the variable sets that clause true, otherwise that location has a one.  Let $c^* = (2\ell_{\epsilon/2}/\epsilon)^{3\ell_{\epsilon/2}}$. This large instance must take at least $2^{n(1-\epsilon-o(1))}$ time.
We can get a lower bound on this instance of $k$-OV in terms of  its input size. The $k$-OV instance requires $N^{k(1-\epsilon-o(1))}$ time.

So $c_\epsilon = c^* = (2\ell_{\epsilon/2}/\epsilon)^{3\ell_{\epsilon/2}}$ which is indeed some fixed constant in terms of $\epsilon$.
\end{proof}


\subsection{How Hard is Counting k-XOR on average?}
In this section we will argue for the average-case hardness of $\oplus k$-XOR from worst case $k$-XOR, OV, and $k$-SUM. 

\begin{lemma}
Let $P_q$ be the problem of solving $\oplus$\ckxor~drawn from the uniform average-case distribution with $g$ sets of vectors of length $b$. Let $q = 1-\frac{2^{-kg}}{3}$ for the rest of this lemma. Additionally we restrict $kg = o(\lg(n)/\lg\lg(n))$ for the rest of this lemma. 

If an $\oplus (SUM,n,k,b,g) \rightarrow (XOR, n,k,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q}$ requires $n^{\lceil k/2 \rceil-o(1)}2^{-kg}$ time if $gb = \gamma(k)k\lg(n)$ and the $k$-SUM hypothesis is true. 

If an $\oplus (OV,n,k,b,g) \rightarrow (XOR, n,k,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q}$ then $P_q$ requires $n^{k (1-\epsilon)-o(1)}2^{-kg}$ time if $gb = c_\epsilon \gamma(k) \lg(n)$ for some fixed constant $c_\epsilon$ if SETH is true. 

If an $\oplus (OV,n,k,b,g) \rightarrow (XOR, n,k,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q}$ requires $n^{\Theta(k)}2^{-kg}$ time if $gb = \gamma(k)kc\lg(n)$ for some fixed constant $c$ if ETH is true.

The $P_q$ problem requires $n^{\lceil k/2 \rceil-o(1)}2^{-kg}$ time if $gb = k \lg(n)$ if the $k$-XOR hypothesis is true. 

\label{lem:FXORfromNormalVerisons}
\end{lemma}
\begin{proof}
For the first three statements we will use Lemma 
\ref{lem:selfReductionsWithbg}. Then we use the definition of the reduction from Definition \ref{def:bgReduction}. Then apply Theorem \ref{thm:frameworkImprovement}. 

The last statement uses Lemma \ref{lem:selfReductionsWithbg} with Theorem \ref{thm:frameworkImprovement}.
\end{proof}

We will give an explicit distribution from which we are drawing our average-case instances of $k$-XOR.

\begin{definition}
We define the distribution $D_{XOR}(k,n,b,g)$ to be a distribution over inputs to $gk$-XOR. This input is generated by taking uniformly random instances of $\oplus$\ckxor~with $k$ lists of $n$ factored vectors where each factored vector is made up of $g$ sets of $b$ length vectors and then applying the reduction from Theorem \ref{thm:factoredToUnfactored}.  
Note that input sizes of instances drawn from $D_{XOR}(k,n,b,g)$ are $N= n 2^b g k$. 
\end{definition}

Now we will go from factored to unfactored XOR. 

\begin{lemma}
Let $P_{q,K,N,b,g}$ be the problem of solving $\oplus K$-XOR~drawn from $D_{XOR}(k,n,b,g)$. Where $N= n 2^b g k$ and $K=gk$. Let $q = 1-\frac{2^{-k}}{3}$ for the rest of this lemma. Additionally we restrict $K=kg = o(\lg(n)/\lg\lg(n))$ for the rest of this lemma. 

If an $\oplus (SUM,n,k,b,g) \rightarrow (XOR, n,k,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q,K,N,\lg(n),\gamma(k)k}$ requires $n^{\lceil k/2 \rceil-o(1)}2^{-kg}$ time if the $k$-SUM hypothesis is true. 

If an $\oplus (OV,n,k,b,g) \rightarrow (XOR, n,k,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q,K,N,\lg(n),\gamma(k)kc_\epsilon}$ requires $n^{k (1-\epsilon)-o(1)}2^{-kg}$ time for some fixed constant $c_\epsilon$ if SETH is true. 

If an $\oplus (OV,n,k,b,g) \rightarrow (XOR, n,k,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q,K,N,\lg(n),\gamma(k)kc}$ requires $n^{\Theta(k)}2^{-kg}$ time for some fixed constant $c$ if ETH is true.

The $P_{q,K,N,\lg(n),\gamma(k)k}$ problem requires $n^{\lceil k/2 \rceil-o(1)}2^{-kg}$ time if the $k$-XOR hypothesis is true. 

\label{lem:XORModularLemma}
\end{lemma}
\begin{proof}
For each of these statements we start by using Lemma \ref{lem:FXORfromNormalVerisons} to show hard average case $\oplus$\ckxor~is from the relevant hypotheses. Then we apply Theorem  \ref{thm:factoredToUnfactored} to go from the factored version to un-factored. By definition running the uniform distribution of \ckxor~through our reduction results in $D_{XOR}(k,n,b,g)$. Given the resulting versions we pick $b=\lg(n)$.
\end{proof}


Now we will plug in our best existing reductions to get the lower bounds. 

\begin{theorem}
Let $P_{q,K,N,b,g}$ be the problem of solving $\oplus K$-XOR~drawn from $D_{XOR}(k,n,b,g)$. Where $N= n 2^b g k$ and $K=gk$, note that $N$ is the input size to the $\oplus K$-XOR problem. Let $q = 1-\frac{2^{-k}}{3}$ for the rest of this lemma. Additionally we restrict $K=kg = o(\lg(n)/\lg\lg(n))$ for the rest of this lemma.

If the $k$-SUM hypothesis is true then
$P_{q,K,N,\lg(n),k^2}$ requires at least $N^{\lceil k^{1/3}/2 \rceil/2-o(1)}$ time. 

If ETH is true then for some fixed constant $c$
$P_{q,K,N,\lg(n), k c}$ requires $N^{\Omega(k^{1/3})}$ time. 

If the $k$-XOR hypothesis is true then the $P_{q,K,N,\lg(n),\gamma(k)k}$ problem requires at least  $N^{\lceil \sqrt{k}/2 \rceil/2-o(1)}$ time. 
\label{lem:XORonAverage}
\end{theorem}
\begin{proof}
In all of the cases above we have $N=n^2$ and $K=kg$, though the value of $g$ changes. We will go through each case starting with the corresponding statements from Lemma \ref{lem:XORModularLemma} and then transform the statements into the new input sizes and parameters. 

We start from Lemma \ref{lem:XORModularLemma} if an $\oplus (SUM,n,k,b,g) \rightarrow (XOR, n,k,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q,K,N,\lg(n),\gamma(k)k}$ requires $n^{\lceil k/2 \rceil-o(1)}2^{-kg}$ time if the $k$-SUM hypothesis is true. Also note that  an $\oplus (SUM,n,k,b,g) \rightarrow (XOR, n,k,kb,g)$ reduction exists which takes $n$ time from Theorem \ref{thm:ovXORsumFromAny}. So $N=n^2$ and $K=k^3$. So we can say that the lower bound is $N^{\lceil k^{1/3}/2 \rceil/2-o(1)}$ time. 

We start from Lemma \ref{lem:XORModularLemma} if an $\oplus (OV,n,k,b,g) \rightarrow (XOR, n,k,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q,K,N,\lg(n),\gamma(k)kc}$ requires $n^{\Theta(k)}2^{-kg}$ time for some fixed constant $c$ if ETH is true. Also note that  an $\oplus (OV,n,k,b,g) \rightarrow (XOR, n,k,kb,g)$ reduction exists which takes $n$ time from Theorem \ref{thm:ovXORsumFromAny}. So $N=n^2$ and $K=ck^3$. Then we can say that there is a lower bound of $N^{\Omega{\sqrt{K}}}$ time. 
We start from Lemma \ref{lem:XORModularLemma} with the $P_{q,K,N,\lg(n),k}$ problem requires $n^{\lceil k/2 \rceil-o(1)}2^{-kg}$ time if the $k$-XOR hypothesis is true. Next note that $N=n^2$ and $K=k^2$. So we have that $P_{q,K,N,\lg(n),k}$ requires $N^{\lceil \sqrt{K}/2 \rceil/2-o(1)}$.
\end{proof}


\subsection{How Hard is Counting k-SUM on Average?}
%A $\oplus (OV,n,k,b,g) \rightarrow (SUM, n+1,k+1,b \lceil \lg(k) \rceil,g)$ reduction exists that takes time $O(ngk2^b)$.
%A $\oplus (XOR,n,k,b,g) \rightarrow (SUM, n+1,k+1,b\lceil \lg(k) \rceil,g)$ reduction exists that takes time $O(ngk2^b)$.
%\label{lem:SUMreductions}
We will start by considering the implications of worst-case fine-grained hypotheses for the hardness of average-case $\oplus$\cksum. We have a much more efficient reduction to $\oplus$\cksum, the overhead in Lemma \ref{lem:SUMreductions} is approximately $\lg(k)$. However, it grows $k$ and $n$ by one, so these increases will propagate through the reduction. 

\begin{lemma}
Let $P_q$ be the problem of solving $\oplus$\cksum[(k+1)]~drawn from the uniform average-case distribution with $g$ sets of vectors of length $b$. Let $q = 1-\frac{2^{-kg}}{3}$ for the rest of this lemma. Additionally we restrict $kg = o(\lg(n)/\lg\lg(n))$ for the rest of this lemma. 

If an $\oplus (SUM,n,k,b,g) \rightarrow (SUM, n+1,k+1,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q}$ requires $n^{\lceil k/2 \rceil-o(1)}2^{-kg}$ time if $gb = \gamma(k)k\lg(n)$ and the $k$-XOR hypothesis is true. 

If an $\oplus (OV,n,k,b,g) \rightarrow (SUM, n+1,k+1,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q}$ then $P_q$ requires $n^{k (1-\epsilon)-o(1)}2^{-kg}$ time if $gb = c_\epsilon \gamma(k) \lg(n)$ for some fixed constant $c_\epsilon$ if SETH is true. 

If an $\oplus (OV,n,k,b,g) \rightarrow (SUM, n+1,k+1,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q}$ requires $n^{\Theta(k)}2^{-kg}$ time if $gb = \gamma(k)kc\lg(n)$ for some fixed constant $c$ if ETH is true.

The $P_q$ problem requires $n^{\lceil (k+1)/2 \rceil-o(1)}2^{-kg}$ time if $gb = k \lg(n)$ if the $k$-SUM hypothesis is true. 

\label{lem:FSUMfromNormalVerisons}
\end{lemma}
\begin{proof}
For the first three statements we will use Lemma 
\ref{lem:selfReductionsWithbg}. Then we use the definition of the reduction from Definition \ref{def:bgReduction}. Then apply Theorem \ref{thm:frameworkImprovement}. 

The last statement uses Lemma \ref{lem:selfReductionsWithbg} with Theorem \ref{thm:frameworkImprovement}.
\end{proof}

We now define the distribution over which we prove hardness for $k$-SUM.

\begin{definition}
We define the distribution $D_{SUM}(k,n,b,g)$ to be a distribution over inputs to $gk$-SUM. This input is generated by taking uniformly random instances of $\oplus$\cksum~with $k$ lists of $n$ factored vectors where each factored vector is made up of $g$ sets of $b$ length vectors and then applying the reduction from Theorem \ref{thm:factoredToUnfactored}.
Note that input sizes of instances drawn from $D_{SUM}(k,n,b,g)$ are $N= n 2^b g k$. 
\end{definition}

Next, we will use the reduction from $\oplus$\cksum~to $K$-SUM to give average-case hardness for $K$-SUM.


\begin{lemma}
Let $P_{q,K,N,b,g}$ be the problem of solving $\oplus K$-SUM~drawn from $D_{SUM}(k+1,n,b,g)$. Where $N= n 2^b g (k+1)$ and $K=g(k+1)$. Let $q = 1-\frac{2^{-k}}{3}$ for the rest of this lemma. Additionally we restrict $K=kg = o(\lg(n)/\lg\lg(n))$ for the rest of this lemma. 

If an $\oplus (XOR,n,k,b,g) \rightarrow (SUM, n+1,k+1,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q,K,N,\lg(n),\gamma(k)k}$ requires $n^{\lceil k/2 \rceil-o(1)}2^{-kg}$ time if the $k$-XOR hypothesis is true. 

If an $\oplus (OV,n,k,b,g) \rightarrow (SUM, n+1,k+1,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q,K,N,\lg(n),\gamma(k)kc_\epsilon}$ requires $n^{k (1-\epsilon)-o(1)}2^{-kg}$ time for some fixed constant $c_\epsilon$ if SETH is true. 

If an $\oplus (OV,n,k,b,g) \rightarrow (SUM, n+1,k+1,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q,K,N,\lg(n),\gamma(k)kc}$ requires $n^{\Omega(k)}2^{-kg}$ time for some fixed constant $c$ if ETH is true.

The $P_{q,K,N,\lg(n),\gamma(k)k}$ problem requires $n^{\lceil (k+1)/2 \rceil-o(1)}2^{-kg}$ time if the $k$-SUM hypothesis is true. 

\label{lem:SUMModularLemma}
\end{lemma}
\begin{proof}
For each of these statements we start by using Lemma \ref{lem:FSUMfromNormalVerisons} to show hard average case $\oplus$\cksum~is from the relevant hypotheses. Then we apply Theorem  \ref{thm:factoredToUnfactored} to go from the factored version to un-factored. By definition running the uniform distribution of \cksum~through our reduction results in $D_{SUM}(k,n,b,g)$. Given the resulting versions we pick $b=\lg(n)$.
\end{proof}

Finally, we will consider the implications in terms of the input sizes and parameters of the generated instances of $K$-SUM. 

\begin{theorem}
Let $P_{q,K,N,b,g}$ be the problem of solving $\oplus K$-SUM~drawn from $D_{SUM}(k+1,n+1,b,g)$. Where $N= n 2^b g k$ and $K=gk$, note that $N$ is the input size to the $\oplus K$-XOR problem. Let $q = 1-\frac{2^{-k}}{3}$ for the rest of this lemma. Additionally we restrict $K=kg = o(\lg(n)/\lg\lg(n))$ for the rest of this lemma.

If the $k$-XOR hypothesis is true then
$P_{q,K,N,\lg(n),k\lceil\lg(k)\rceil}$ requires at least  $N^{\sqrt{K/(8\lg(K))}-o(1)}$ time. 

If ETH is true then for some fixed constant $c$
$P_{q,K,N,\lg(n), \lg(k) c}$ requires $N^{\Omega(\sqrt{K/\lg(K)})}$ time. 

If the $k$-SUM hypothesis is true then the $P_{q,K,N,\lg(n),k}$ problem requires $N^{\lceil (\sqrt{K}-1)/2 \rceil/2-o(1)}$ time. Note that this also implies a lower bound of $N^{(\sqrt{K}-1)/4-o(1)}$ time.
\label{lem:SUMonAverage}
\end{theorem}
\begin{proof}

Here we will convert from $k$ to $K$ and $n$ to $N$. For each statement we will start with the statement from Lemma \ref{lem:SUMModularLemma} and then do this conversion. 

From Lemma \ref{lem:SUMModularLemma} we know that if an $\oplus (XOR,n,k,b,g) \rightarrow (SUM, n+1,k+1,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q,K,N,\lg(n),\gamma(k)k}$ requires $n^{\lceil k/2 \rceil-o(1)}2^{-kg}$ time if the $k$-XOR hypothesis is true. By Lemma \ref{lem:SUMreductions} we have that a $\oplus (XOR,n,k,b,g) \rightarrow (SUM, n+1,k+1,\lceil\lg(k)\rceil b,g)$ reduction exists which takes $n^{o(k)}$ time. So $K= \lceil\lg(k)\rceil k (k+1)$ and note that $\sqrt{2K/\lceil\lg(K)\rceil} \leq k$. Further note that $N=n^2$. Now we can plug in for a value of $N^{\lceil \sqrt{2K/\lceil\lg(K)\rceil}/2 \rceil/2-o(1)}$. To simplify this statement we can instead write our lower bound as $N^{\sqrt{K/(8\lg(K))}-o(1)}$, we loose the ceilings, but get a much simpler and still true statement. 

From Lemma \ref{lem:SUMModularLemma} we know that if an $\oplus (OV,n,k,b,g) \rightarrow (SUM, n+1,k+1,\gamma(k)b,g)$ reduction exists which takes $n^{o(k)}$ time then
$P_{q,K,N,\lg(n),\gamma(k)kc}$ requires $n^{\Omega(k)}2^{-kg}$ time for some fixed constant $c$ if ETH is true. By Lemma \ref{lem:SUMreductions} we have that a $\oplus (OV,n,k,b,g) \rightarrow (SUM, n+1,k+1,\lceil\lg(k)\rceil b,g)$ reduction exists which takes $n^{o(k)}$ time. So $K= \lceil\lg(k)\rceil c k(k+1)$ and note that $\sqrt{K/\lg(K)} = O(k)$. Additionally, $N= n^2$. Now we can give the lower bound as $N^{\Omega(\sqrt{K/\lg(K)})}$.

From Lemma \ref{lem:SUMModularLemma} we know that if the $k$-SUM hypothesis is true then the $P_{q,K,N,\lg(n),\gamma(k)k}$ problem requires $n^{\lceil (k+1)/2 \rceil-o(1)}2^{-kg}$ time.  Here we have $N=n^2$ and $K= (k+1)(k+1)$. So, we can plug in $\sqrt{K}=k+1$ to get a lower bound of $N^{\lceil \sqrt{K}/2 \rceil/2-o(1)}$. Note that this also implies a lower bound of $N^{(\sqrt{K}-1)/4-o(1)}$.
\end{proof}



==> SAT.tex <==
%\xxx{Idea: can we go from the (lots of clauses) SAT instance back to OV? Note that if we pick $\ell >>> k$ then the instance of OV will have $N = 2^{n/k}$ vectors of dimension $D\approx 2^{n/\ell}$. So $D=N^{k/\ell}$, this is a polynomially large dimension, but, it can be an arbitrarily small polynomial. I haven't read the paper that shows hardness for k-SUM (I think it is Ryan William's paper?) but maybe we can make this work there as well even with the large dimension. Additionally, the reduction is less efficient but doesn't break for small $\ell = \omega(1)$. So that should also be in consideration. Anyway, we might be able to get better hardness but for versions of k-OV and k-SUM with really long vectors/numbers.}

In this section we present a reduction from $3$-SAT %\vnote{Is the starting point 3SAT or $k$-SAT? Does it matter?} \anote{It doesn't matter, in a previous version we cared a bit, but now we don't care at all. We just want some constant $k$-SAT. I thought it was clean to stick with the $3$} \vnote{That's good. I would just be consistent with the figure. Maybe  then just change the figure to parity-3-sat?}\mina{will do}
to average-case Parity-CNF-SAT ($\oplus$CNF-SAT, which we will refer to as $\oplus$SAT), and demonstrate an average-case distribution of $\oplus$CNF-SAT which requires $2^{\Omega{(n)}}$ time, where $n$ is the number of variables. %\virgi{Probably want parity cnf sat}
We do this in $4$ steps: In step 1, we reduce $k$-SAT for any constant $k$ to $\ell$-OV, where $\ell$ is a super constant but very small with respect to the size of our problems. Then in step 2 we reduce $\ell$-OV to factored $\ell$-OV, and in step 3 we use the framework of Section \ref{sec:frameworkBetter} to get average-case hardness for our factored $\ell$-OV problem. Finally in step 4 we reduce factored $\ell$-OV to a CNF-SAT instance. See Figure \ref{fig:ethReductionTight}.

%We use the framework of Section \ref{sec:frameworkBetter} to give average-case hardness for factored $\ell$-OV from ETH for some $\ell>0$. Then, we give a reduction from average-case $\ell$-OV to average-case SAT. We get a $2^{\Omega(n)}$ lower bound on an average-case distribution of $\oplus$CNF-SAT (note that this allows large clauses). We use OV as an intermediate step because it improves the efficiency of describing clauses, saving a logarithmic factor in the exponent. However, using OV this way causes our clauses to be very large. Our reduction consists of $4$ steps with step 4 being the main result. See Figure \ref{fig:ethReductionTight} for a depiction of the reduction steps. \mina{What restrictions do we have on $\ell$? Or what $\ell$ do we choose at the end?} \anote{The restriction is just that it is a constant. We will set it to some very large constant (dependant on ETH).}



 %We will start by noting the implied hardness of \ckov[\ell]~from previous work. 

%\subsection{Step 1 and 2: Hardness of \ckov[\ell]~from ETH}

\paragraph{Step 1: From SAT to OV.}
Here we state the reduction from SAT to $\ell$-OV for any $\ell$. 
%\virgi{State that $\ell=O(1)$ and define $\oplus \ell$-OV.}
\begin{theorem} [Reduction from SAT to OV (see e.g. \cite{Williams05})] %One can reduce an instance of $k$-SAT with $n$ variables and $m=O(n)$ clauses to an instance of $\lg{n}$-OV of size $O(2^{n/\lg{n}})$ in $O(\lg{(n)}2^{n/\lg{n}}m)$ time.
Consider $k$-SAT with $n$ variables and $m=O(n)$ clauses. 
If an algorithm exists for $\oplus \ell$-OV on $N$ zero-one vectors each of dimension $D$ which runs in time $T(N,D,\ell)$, then there is an algorithm for $\oplus k$-SAT which runs in $O(T(2^{n/\ell}, m,\ell) + 2^{n/\ell}m)$ time.
\label{thm:SATtoOV}
\end{theorem}
\begin{proof}
The reduction from \cite{Williams05} takes a single instance of $k$-SAT and turns it into a single instance of $2$-OV. The reduction easily generalizes to a fine-grained reduction to $\ell$-OV for any $\ell\geq 2$ (see discussion in \cite{virgiSurvey}). To do this we split the set of variables in the $k$-SAT instance into $\ell$ groups of size $n/\ell$. Then we enumerate all $2^{n/\ell}$ possible settings of the variables in each set, we form one partition in our $\ell$-OV instance for each of the $\ell$ sets. For each possible setting of a variable in each set we form a vector with one bit per clause. The bit is set to zero if the variable setting causes the clause to be set true. The bit is otherwise set to $1$. Now consider a set of $\ell$ vectors,$v_1,\ldots, v_\ell$, one from each partition, such that $\forall i$ $\exists j$ $v_j[i]=0$, where $v_j[i]$ is the $i$th bit of $v_j$. Note that this corresponds to a setting of the variables that satisfies the original formula. In fact, this is a one to one correspondence. The number of solutions of the generated $\ell$-OV instance equals the number of solutions of the original $k$-SAT instance. This reduction takes $O(2^{n/\ell}m)$ time, which is the size of the input of the $\ell$-OV instance.
\end{proof}
\paragraph{Step 2: From OV to factored OV.}
Step 2 in our chain of reductions comes from \cite{factoredProblems} that presents a reduction from $\ell$-OV to its factored version \ckov[\ell]. 

\begin{theorem}
Let $\ell=o(\lg{N})$. In $\tO(N)$ time, one can reduce an instance of size $N$ of $\oplus\ell$-OV with vectors of dimension $d$ with a single call to an instance of size $\tO(N)$  of $\oplus$\ckov[\ell]$(b,g)$ for any $g,b>0$ where $gb=d$.%\vnote{What is $k$? perhaps you mean $\ell$?}
\label{thm:DLWunfactoredToFactored}
\end{theorem}
\begin{proof}
\cite{factoredProblems} had the assumption that $\ell$ is a constant, but for small super constants this is still correct with the same proof. We take each vector from the $\ell-OV$ instance, and break it into $g$ subvectors of length $b$, and this turns the vector in to a factored vector, where each of the $g$ sets of the factored vector only has one $b$-bit vector in it. This takes linear time in the size of the input which is $O(\ell N)=\tO(N).$
\end{proof}


%Next we will use the framework to show hardness for the uniform average-case of $\oplus$\ckov[\ell].
\paragraph{Step 3: Average-case hardness of $\oplus$\ckov[\ell]}
Here we prove the average-case hardness of 
$\oplus$\ckov[\ell]$(N,b,g)$. We will do this using the framework in Section \ref{sec:frameworkBetter}. By Lemma \ref{lem:factored-gdlp}, a \ckov[\ell]$(N,b,g)$ instance has a $\ell g$-degree polynomial if we choose $b=o(\log{N})$. This result is proved in \cite{factoredProblems} for constant values of $\ell$, however since we want to use super constant values for $\ell$ we provide the proof for completeness.%\vnote{This result is essentially in DLW, but you give a simpler proof? Do you get better parameters? If yes, highlight it. In any case, give credit to DLW.}


%\mina{$b$ must have some bound: we will have $g2^b$ variables and we want it to be $o(N)$?? So $b=o(log{n})=o(n/\ell)$?}
%\begin{lemma}\label{lem:gldpForParOV} 
%If $P$ is the problem $\oplus$\ckov[\ell]$(b,g)$, factored $\ell$-OV with $g$ sets each of $b$ length strings, then there exists a function $f_{F\ell OV}$ which is a good $\ell g$-degree polynomial for $P$. 
%\vvnote{It's a bit hard to parse these type of statements. Being more verbose is better in this case.}
%\end{lemma}
%\begin{proof}
%Let us first give a general polynomial called $f_{\ell\text{-}func}(\vec{X})$  from \cite{factoredProblems}. They start by defining $S_f$ to be the subset of $\ell$ tuples of vectors in  $\{0,1\}^b$ such that $f(s_1,\ldots,s_{\ell})=1$ (for some function $f$ over $k$ strings of length $b$.
%$$f_{\ell\text{-}func}(\vec{X}) = \sum_{v_1 \in V_1, \ldots, v_\ell \in V_\ell} \left( \prod_{i \in [0,g-1]} \left( \sum_{(s_1,\ldots, s_{\ell})\in S_f}  x_{v_1[i]}(\vec{s_1}) \cdots x_{v_k[i]}(\vec{s_{\ell}}) \right) \right).$$
%Let $f_{F\ell OV}(\vec{X})$ be $f_{\ell\text{-}func}(\vec{X})$ where $f$ returns $1$ if $(s_1,\ldots, s_{\ell})$ are $\ell$ orthogonal vectors.
%Next we use Lemma 3.1 from \cite{factoredProblems} \mina{probably put the lemma here as well}. This notes that the function $f_{F\ell OV}$ is a good low-degree polynomial  of degree $\ell g$.
%\end{proof}
Using our parity framework Theorem \ref{thm:BetterFrameworkParity}, we have the following result.

\begin{theorem}
Consider the factored $\ell$-OV problem $\oplus$\ckov[\ell]$(N,b,g)$, where $b=o(\lg{N})$ and $g\ell=o(\lg(N))$. %\vnote{Sounds like $g\ell$ has to be $o(\log N)$. See comments below.}
%Let $P$ be the problem of uniform average-case $\oplus$\ckov[\ell]~on $N$ factored vectors each of $g$ sets with $b$ length vectors.
If an algorithm $\alg$ exists for $\oplus$\ckov[\ell]$(N,b,g)$ which takes $T(N,b,g,\ell)$ time and succeeds with probability $1-2^{-g\ell-3}$ then there exists an algorithm for worst-case $\oplus$\ckov[\ell]$(N,b,g)$~which runs in time $\tilde{O}(N+T(N,b,g,\ell))$.%\vnote{The run time doesn't compute: It should be at least the number of instances times $T(N,b,g,\ell)$ and the number of instances is some $o(N)$... not sure how you get this number.} Mina:gl = o(lgN) so it should be good now.
\label{thm:FOVisHard}
\end{theorem}
\begin{proof}
Note that Theorem \ref{thm:BetterFrameworkParity} (which is proved in section \ref{sec:frameworkBetter}) %\vnote{Theorem reference should not be to the intro}\andrea{We are using re-statable so that all instances of the same thm have the same number. Is the section reference an okay solution?} 
reduces one instance of $\oplus$\ckov[\ell]$(N,b,g)$ to $2^{g\ell}-1=o(N)$ %\vnote{I don't see how this is $o(N)$. $g\ell$ could be $\Omega(\log N)$ with the current setting of parameters, no?} 
instances of  $\oplus$\ckov[\ell]$(N,b,g)$ where the input is taken from the uniform distribution\footnote{i.e. the $b$-bit vectors in factored vectors are taken uniformly from $\{0,1\}^b$}. If such an algorithm $\alg$ exists, then there is an algorithm for worst-case $\oplus$\ckov[\ell]$(N,b,g)$ that runs in 
$O(2^{g\ell}(N2^bg+T(N,b,g,\ell))$ time. Since $b,g,\ell=o(\lg{N})$, we have $2^{b}=o(N)$ and $2^{g\ell}=o(N)$, %\vnote{same comment as above; I don't see why this is $o(N)$.}
and so we get the stated running time.  
\end{proof}
%\begin{proof}
%We use the reduction from Theorem \ref{thm:BetterFrameworkParity} combined with Lemma \ref{lem:gldpForParOV}.
%\end{proof}

%Note that when $b=o(\log{N})$ and $g=o(N)$, the above running time is $\tilde{O}(2^{g\ell}(N+T(N,b,g)))$. 

Finally, we present a reduction from $\oplus$\ckov[\ell]~to $\oplus$SAT. This will imply the average-case hardness of $\oplus$SAT on the distribution of inputs induced by running the reduction starting from the uniform average-case distribution of $\oplus$\ckov[\ell] instances. %\virgi{Is $\oplus$\ckov[\ell] defined somewhere?}

\subsection{Step 4: From factored OV to SAT}

In the next theorem, we give a reduction from $\oplus$\ckov[\ell]~to $\oplus$SAT which is our main result in this section. 

\begin{theorem}
Let $I$ be an instance of $\oplus$\ckov[\ell]$(N,b,g)$ where $b,g\ell=o(\lg{N})$. %factored $\ell$ OV ~with $\ell$ partitions each with $2^{n/\ell}$ factored vectors each formed with $g$ sets of $b$-length zero-one vectors. 
There exists a reduction in $\tilde{O}(N)$ time which transforms $I$ into an instance $I'$ of $\oplus$SAT with $\hat{n} = \ell \lg{N} + \ell bg$ variables and $\hat{m}\leq N2^{b} g \ell + bg$ clauses. 
\label{thm:fkov-sat}
\end{theorem}
\begin{proof}
%Let $N =2^{n/\ell}$ to make our math cleaner. 
We want to encode a $F\ell$-OV instance in a SAT instance, so we have to determine what we want to encode from the $F\ell$-OV instance. In an $F\ell-OV$ instance we take one factored vector from each of the $\ell$ partitions, and then for each factored vector and for each $j=1,\ldots,g$, we pick a $b$-length vector in the $j$th set of this factored vector, and see if the vectors selected from the $j$th sets are orthogonal for all $j$. To encode this in a SAT instance, the general idea is to have indicator variables, indicating the choice of the $\ell$ factored vectors. 

Suppose that for each $i=1,\ldots,\ell$, the factored vectors in partition $i$ are labeled from $1$ to $N$. The variables $\vec{x}_i = (x_{i,0}, \ldots, x_{i,\lg(N)-1})$ indicate the label of the factored vector in partition $i$ that we are picking. For example for $N=4$, $\vec{x}_i = (1,0)$ indicates the factored vector in partition $i$ with label $2$. 

To encode the choice of the $b$-length vector in a chosen factored vector, we define variables $\vec{y}_{i,j} = (y_{i, j, 1}, \ldots, y_{i,j,b})$ which indicate the $b$-bit vector selected from the $j^{th}$ subset of the factored vector from the $i^{th}$ partition. Note that $\vec{y}_{i,j}$s are the actual vectors whereas $\vec{x}_{i}$s are labels of the factored vectors.

Now we have to enforce the constraints of the $F\ell-OV$ instance on these variables using CNF clauses. 
If $a\in [0,N-1]$ let $C(\vec{x}_i \neq a)$ return a clause which is false only if the bits $(x_{i,0}, \ldots, x_{i,\lg(N)-1})$ represent the number $a$. For example if $N=8$ and $a=5$ then the representation of $5$ is $101$. The clause would be $ C(\vec{x}_i \neq a)=(\lnot{x}_{i,0} \vee x_{i,1} \vee \lnot{x}_{i,2})$.  More formally, if $a_t$ is the $t^{th}$ bit of $a$, we have that $C(\vec{x}_i\neq a)$ is the OR of $\log{N}$ clauses, where the $t^{th}$ clause is $x_{i,t}$ if $a_t=0$ and it is $\lnot{x_{i,t}}$ otherwise. 

Additionally if $s \in \{0,1\}^b$ let $C'(\vec{y}_{i,j} \neq s)$ return false only if the bits $(y_{i, j, 1}, \ldots, y_{i,j,b})$ represent the string $s$. This can be defined analogously to $C(\cdot\neq \cdot)$.%\xxx{This can be explained better. I am not sure how to write it cleanly. But we want $ C(\vec{x}_i \neq a)$ to be the obvious thing where any bit in $a$ that is a zero we leave as a non-negated literal and any bit in $a$ that is a one we leave the corresponding variable negated.}

Now we can discuss our formula $\phi$. In the $F\ell-OV$ instance, let $\vec{v}_{i,a}$ be the $a^{th}$ factored vector from partition $i$, and recall that $\vec{v}_{i,a}[j]$ is the $j^{th}$ set of $b$-length vectors in the factored vector $\vec{v}_{i,a}$. For all $i\in [1,\ell]$, for all $a\in [0,N-1]$, for all $j\in [1,g]$, and for all $s \in \{0,1\}^b \setminus \vec{v}_{i,a}[j]$ (so for all strings not in the $j^{th}$ set of $\vec{v}_{i,a}$) we add the clause
$$ C(\vec{x}_i \neq a) \vee C'(\vec{y}_{i,j} \neq s)$$
to $\phi$. Note that these clauses enforce that our choices of $\vec{x}_i$ and $\vec{y}_{i,j}$ are consistent with each-other and the input.
This is because the set of clauses over all $s$ above ensures that whenever $x_i=a$, we must have $\vec{y}_{i,j}\in v_{i,a}[j]$.
% This is because the only time that this clause returns false is when $\vec{x}_i$ encodes $a$ (so we have chosen the $a^{th}$ vector from partition $i$, i.e. $\vec{v}_{i,a}$), and that the $b$-length vector supposedly chosen from the $j^{th}$ subset of this vector is actually not in this set. \virgi{Isn't it clearer to say that the set of clauses over all $s$ above ensures that whenever $x_i=a$, $y_{i,j}$ must equal $v_{i,a}[j]$?}

Finally, we need to add clauses to $\phi$ that check that the values in $\vec{y}_{i,j}$ represent orthogonal vectors.  For all $j\in [1,g]$ and for all $p \in [1,b]$ we add the clause 
$$(\lnot{y}_{1,j,p} \vee \lnot{y}_{2,j,p} \vee \ldots \vee \lnot{y}_{\ell,j,p})$$
to $\phi$. Note that this clause is checking that there is at least one zero amongst all of the $p^{th}$ bits of all $\ell$ selected strings from the $j^{th}$ sets of our factored vectors. If this is true for all bits across all sets, then the vectors are orthogonal and represent a single solution.  %\virgi{The bars above the variables are hard to see. Why not use $\lnot$?}

Now we count the number of variables. There are $\ell\lg(N)$ $x$ variables and $\ell b g$ $y$ variables. This gives a total of $\hat{n} = \ell \lg(N) + \ell b g $%= n +\ell bg$
 variables. To count the number of clauses, note that in our first set of added clauses there are at most $N2^bg\ell$, in our second set there are $bg$, giving a total of $\hat{m} \leq N2^bg\ell+bg$. To compute the running time, note that the $C(\vec{x}_i\neq a)$ and $C'(\vec{y}_{j,i}\neq s)$ take $O(\lg{N})$ and $O(b)$ to create respectively, for each $i,j,s,a$. So each clause takes $O(b+\lg{N})$ to make, and so the running time of the reduction is $O(\hat{m}(b+\lg{N}))=\tilde{O}(N)$.

So any setting of all $x$ and $y$ variables that results in a satisfiable formula corresponds to a single solution to the original \ckov[\ell]~instance. Thus, a  solution to this $\oplus$SAT problem solves the original $\oplus$\ckov[\ell]~instance. This proves our statement.
\end{proof}

\subsection{Average-Case hardness of $\oplus$SAT}

Using our 4 step reduction from worst-case $\oplus$SAT to average-case $\oplus$SAT, we are going to define the distribution of $\oplus$SAT that we will show is hard. %\mina{Can we describe the distribution without using the reduction or OV?} \anote{I am not sure how to describe it without that.}

\begin{definition} 
Let $D^{N}_{\oplus SAT(b,g,\ell)}$ be the distribution generated by sampling the input from the uniform distribution of $\oplus$\ckov[\ell]$(N,b,g)$ and running the reduction from Theorem \ref{thm:fkov-sat}. Note that the instances generated from this distribution will have $\hat{n}=\ell \lg{N}+\ell bg$ variables and $\hat{m}\le N2^bg\ell+bg$ clauses.
\end{definition}

%\begin{definition} 
%Let $D$ be the distribution generated by sampling the input from the uniform distribution of $\oplus$\ckov[\ell]$(N,\sqrt{N},\sqrt{N})$ for $\ell=\lg{N}$ and running the reduction from Theorem \ref{thm:fkov-sat}. Note that the instances generated from this distribution will have $\hat{n}=\lg{N}(N+\lg{N}) $ variables and $\hat{m}\le N2^bg\ell+bg$ clauses.

%\end{definition}

Finally, we will show that $\oplus$SAT is hard on average.

%\mina{In the Theorem statement below If $bg=\Theta(n)$, then $\hat{n}=O(\ell n)$ so we can simplify it? We have TOO many variables in the theorem/proof below, should simplify as much as we can. Or we can put a simplified version here and put a more complicated/accurate one in the appendix.}

%\xxx{We can maybe re-frame this as lemma and choose $b=g=\sqrt{m}$ arbitrarily. We don't really care about the exact choice, and this will clean up our statements. }

%\xxx{From discussion with Mina: This should probably be set as a lemma, and we should make a theorem where $\ell = \lg(n)$ and $b=g=\sqrt{m}= O(\sqrt{n})$. The theorem then looks like a reasonable readable statement in English. The lemma has the generality to be used later if we need or want it.}
%\mina{for the sake of the probability, $g$ should as small as possible.}
%\xxx{TODO for andrea: make clear in theorem and lemma statements what the cost of the reduction is. So e.g. we start with $n$ vars and $m$ clauses we have a reduction that runs in $R(n,m)$ to produce an average case instance (or several average-case instances) with $V(n,m)$ variables and $C(n,m)$ clauses.}
%\mina{We need a statement noting that if $I$ has $\hat{n}$ variables and $\hat{m}$ clauses, then it cannot be solved in $poly(\hat{m})2^{o(\hat{n})}$ time. Maybe we can keep this and have Theorem \ref{thm:averagecaseSAT}}

\begin{theorem}
Let $\ell=\lg(\lg(\lg(n)))$.  Let $g= o(n/\ell)$ and $b=o(n)$ such that $bg =\Theta(n)$. 
%\vnote{Sounds like $g\ell$ has to be $o(n)$.} \andrea{yeah, I think this was changed recently. We used to have $\ell$ constant.}
%Let $\hat{m}=2^{n/\ell+b}g\ell +bg$. 
% \mina{define $\ell$?} good point
%Let $I$ be  an instance of $\oplus$SAT that is drawn from $D^{2^{n/\ell}}_{\oplus SAT(b,g,\ell)}$, so $I \sim D^{2^{n/\ell}}_{\oplus SAT(b,g,\ell)}$. Let $\hat{n}$ be the number of variables and let $\hat{m}$ be the number of clauses in the $\oplus$SAT instance. 
%If an algorithm, $\alg$ exists for all constant $\ell>2$ such that on $I \sim D^{2^{n/\ell}}_{\oplus SAT(b,g,\ell)}$,  $\alg(I)$ returns the parity of the number of satisfying assignments to $I$ with probability $1-2^{-g\ell-2}$ in time $poly(\hat{m}) \cdot 2^{o(n)}$ then ETH is false. 
If an algorithm $\alg$ exists such that on $I \sim D^{2^{n/\ell}}_{\oplus SAT(b,g,\ell)}$,  $\alg(I)$ returns the parity of the number of satisfying assignments to $I$ with probability $1-2^{-g\ell-3}$ in time $poly(\hat{m})2^{o(\hat{n})}$ then rETH is false. 
\label{thm:AvgCaseHardSAT}
\end{theorem}
\begin{proof}
Assume that rETH is true.
Consider an instance of $\oplus 3$-SAT with $n$ variables and $m=O(n)$. Note that rETH and Lemma \ref{lem:decisionToParity} imply that this problem requires $2^{\Omega(n)}$ time. We use our $4$ step reduction below.
\begin{itemize}
    \item Step 1: We apply Theorem \ref{thm:SATtoOV} to reduce the $\oplus 3$-SAT instance to an instance of $\oplus \ell$-OV with $N=2^{n/\ell}$ vectors each of dimension $D = m$, in $O(2^{n/\ell}m)=2^{o(n)}$ time.
    \item Step 2: We reduce from $\oplus \ell$-OV to $\oplus$\ckov[\ell]$(2^{n/\ell},b,g)$ using Theorem \ref{thm:DLWunfactoredToFactored} in $poly(n)2^{o(n)}=2^{o(n)}$ time.
    \item Step 3: We use Theorem \ref{thm:FOVisHard} to reduce this instance of $\oplus$\ckov[\ell]$(2^{n/\ell},b,g)$ to $2^{g\ell}-1=2^{o(n)}$ uniform average-case instances of $\oplus$\ckov[\ell]$(2^{n/\ell},b,g)$, in time $2^{o(n)}$ since the size of each instance is $2^{o(n)}$. %to prove the that uniform average-case $\oplus$\ckov[\ell]$(b,g)$ of size $2^{n/\ell}$ requires $2^{\Omega(n)-\ell g}$ time with probability $1-2^{-g\ell-2}$.
    \item Step 4: We apply Theorem \ref{thm:fkov-sat} on all the $\oplus$\ckov[\ell]$(2^{n/\ell},b,g)$ instances. For each, we produce an instance of $\oplus$SAT via our reduction from an instance of $\oplus$\ckov[\ell]$(2^{n/\ell},b,g)$, in $2^{o(n)}$ time. %with $g$ groups of $b$ length strings. 
    Thus, by definition, producing an instance of $\oplus$SAT drawn from $D^{2^{n/\ell}}_{\oplus SAT(b,g,\ell)}$. 
    
\end{itemize}
  %factored vectors of $g$ subsets each of $\{0,1\}^b$ where $bg = D = m$.
 %, uniform average-case $\oplus$\ckov[\ell]~with $N''=2^{n/\ell}$ factored vectors each with $g$ subsets of $\{0,1\}^{b}$. 
 
Now to prove the theorem, suppose that such an algorithm $\alg$ exists with running time $poly(\hat{m})2^{o(\hat{n})}=2^{o(n)}$ that returns the parity of satisfying assignments of SAT instances drawn from $D^{2^{n/\ell}}_{\oplus SAT(b,g,\ell)}$ with success probability $1-2^{-g\ell -2}$. We start from Step $4$ and see what this results for each step.
\begin{enumerate}
    \item Step 4: By Theorem \ref{thm:fkov-sat}, the existence of $\alg$ means that there is an algorithm for average case $\oplus$\ckov[\ell]$(2^{n/\ell},b,g)$ with uniform input with success probability $1-2^{-g\ell -3}$ in $2^{o(n)}$ time. Note the success probability does not degrade because this reduction step is a single-call worst-case reduction. %\vnote{I am not sure how you get this success probability. Are all the $2^{o(n)}$ instances produced by the reduction independent? I assume not, so applying the union bound should give you success probability $1-2^{o(n)}/2^{g\ell+3}$. This is bothersome because it seems to me --- see above --- that $g\ell$ has to be $o(n)$ too.}\mina{tnis probability comes directly from the framework theorem after a union bound}
    \item Step 3 and 2: Using Theorem \ref{thm:FOVisHard}, there is a randomized algorithm for worst-case $\oplus$\ckov[\ell]$(2^{n/\ell},b,g)$ in $poly(n)O(2^{n/\ell}+2^{o(n)})=2^{o(n)}$, and thus an algorithm in the same running time for $\ell$-OV of size $2^{n/\ell}$. This is the step where we make $2^{g\ell}$ calls to our average-case  $\oplus$\ckov[\ell]$(2^{n/\ell},b,g)$ solver, and by a union bound, we have a randomized worst-case algorithm with success probability $7/8$. %This can be boosted using traditional randomized algorithms methods. 
    \item Step 1: Finally, this gives us an algorithm for $\oplus3$-SAT in $2^{o(n)}$ time which succeeds with probability greater than $2/3$, which by Lemma~\ref{lem:decisionToParity} refutes rETH.
\end{enumerate}
This proves the theorem. Note that for $\ell$ we can put any small increasing function of $n$, since we only need $\frac{n}{\ell}=o(n)$. So, $\ell$ could be even more slow growing than the version we gave here.  % \vnote{same comment about $\ell$ vs $g\ell$.}
%This instance of $\oplus$SAT will have $\hat{n} = n + \ell bg = n + \ell m$ and $\hat{m} =  2^{n/\ell +b}g+bg$. 
%The total cost, in time, of this series of reductions is $O(2^{\ell g + b + n/\ell})$. \mina{reduction time needs more clarification}
%If ETH is true then  $3$-SAT with $n$ variables and $m=O(n)$ requires $2^{n (1/c -o(1))}$ time for some constant $c$.
%Assume, for the sake of contradiction, that an $O(\hat{m}^p 2^{o(\hat{n})})$ algorithm existed for $\oplus$SAT drawn from $D^{2^{n/\ell}}_{\oplus SAT(b,g,\ell)}$ for all constant $\ell$ which succeeds with probability $1-2^{-\ell g-2}$.
%Choose $\ell = 2cp$ and choose $g$ and $b$ to both be $\omega(1)$ and $o(n)$. We have $bg = m = O(n)$, so any choice of $b \in \omega(1) \cup o(n)$ implies that $g \in \omega(1) \cup o(n)$ as well. Given these restrictions we get $\hat{n} = \Theta(n)$ and the reduction overhead is $O(2^{n/(2pc)+o(n)})$ time. Now, a $\hat{m}^p 2^{o(\hat{n})}$ time algorithm would imply an $O(2^{n/(2pc)+o(n)} \cdot 2^{n/(2c) +o(n)} \cdot 2^{o(n)})$ time algorithm for worst-case $3$-SAT, violating ETH. 
%Thus, by contradiction, no $poly(\hat{m})2^{o(\hat{n})}$ time algorithm exists for $\oplus$SAT. 
\end{proof}


\sathardness*
\begin{proof}
In Theorem \ref{thm:AvgCaseHardSAT} let $g=\lg(\lg(n))/\ell$ and $b=n/g$. %\xxx{Andrea please check if this substitution is okay}. Andrea: LGTM!
The distribution $D$ is going to be $D^{2^{n/\ell}}_{\oplus SAT(b,g,\ell)}$ for $\ell = \lg(\lg(\lg(n)))$.
\end{proof}


%\begin{reminder}{Corollary \ref{cor:averagecaseSAT}}
%\begin{corollary}
%\label{thm:averagecaseSAT}
%For any $n$ and $m=O(n)$, there exist $\hat{n}=O(n)$ and $\hat{m}=O(2^{\Theta(\sqrt{n}})$ and a particular, efficiently samplable, distribution $D$ over SAT instances with at most $\hat{n}$ variables and at most $\hat{m}$ clauses, such that the average case parity SAT over $D$ cannot be solved in $\poly(\hat{m})2^{o(\hat{n})}$ with probability $1-2^{-\omega(\sqrt{n})}$ assuming ETH.
%\end{reminder}
%\end{corollary}
%\begin{proof}
%We will plug in the values of $b=g=\sqrt{m}=\Theta(\sqrt{n})$ into Theorem \ref{thm:AvgCaseHardSAT}. As we leave the distribution $D$ in our theorem statement unspecified we can set it to $D^{2^{n/\ell}}_{\oplus SAT(b,g,\ell)}$ where $\ell=2cp$ as defined in \ref{thm:AvgCaseHardSAT}. So, given our settings the distribution we pick is  $D^{2^{n/\ell}}_{\oplus SAT(\sqrt{m}, \sqrt{m},\ell)}$ when $\ell=2cp$.
%\end{proof}

%\andrea{We can consider adding a non-corollary, where we pick values of $b$ and $g$ such that $\ell$ can be non-constant which would allow us to clean up the whole setting $\ell$ later and issues with some unknown values that cause us to need the algorithm to work on many distributions. }

%%%%% We can get a lower bound of $2^{\Omega(\sqrt{n})}$...but this is just like the previous result! We want something more efficient to be impressive. 
%\subsection{Average-Case hardness of $\oplus$4-SAT}
%In this section we give a less efficient reduction which gives hardness for $\oplus4$-SAT on average. We increase the number of variables to decrease the size of clauses needed. The core idea is this: what if we had a variable in our formula to indicate the choice of each possible factored vector and for every factored vector which of the $2^b$ choices is being selected for each of the $g$ sets. So, this gives us a total of $\ell 2^{n/\ell} + \ell g 2^b$ variables. Note that if we pick $\ell = g = n/\alpha(n)$ for some small function $\alph(n) = \omega(1)$ then this works out to $O(n^2 2^{O(\alpha(n))})$ variables. 

==> SATtoOV.tex <==
%\mina{Maybe we should mention this after we section 7?} \andrea{moved!}
In this section we will show hardness for $k$-OV from the average-case $\oplus SAT$ problem described in Section \ref{sec:avgCaseSat}. There will be three important differences from this reduction and the reduction in Section \ref{sec:ac-kov}. The first difference is that the distribution we show hard is different in these two cases. The second difference is that in this case the vectors have larger dimension: if the $k$-OV instance has $N$ vectors in each list, then the dimention is $o(N)$ instead of $O(\lg{N})$. Moreover $k$ is not a constant (although any small super constant would work, we set $k=o(\lg(\lg(\lg(N)))$). The third and final crucial difference is that in this section we will show a distribution average-case $\oplus k$-OV is $N^{\Theta(k)}$ hard whereas in Section \ref{sec:ac-kov} we give a distribution on which average-case $\oplus k$-OV is $N^{\Omega(\sqrt{k})}$ hard. So, in this section we show stronger hardness but with much longer vectors. 

The reduction will follow from applying the standard $\oplus$SAT to $\oplus k$-OV reduction. 

We start by describing a standard  reduction from SAT to $k$-OV. The following lemma is similar to Lemma \ref{lem:dimensionReductionETH}.

\begin{lemma}
Given an instance of $\oplus$SAT with $n$ variables and $m$ clauses there is a reduction which runs in time $O(k2^{n/k}mn)$ which produces a single instance of $\oplus k$-OV with $k$ lists of $N=2^{n/k}$ vectors each of dimension $D=m$. 
\label{lem:SATtoOVWorstCase}
\end{lemma}
\begin{proof}
%This is the standard reduction for $k$-OV. 
Given an instance of $\oplus$SAT, we create $k$ lists of vectors as follows: We split the $n$ variables of $\oplus$SAT into $k$ groups of $n/k$ variables each. Each group will be used to form a list of size $N=2^{n/k}$. For the $i^{th}$ group of variables $S_i$ we consider every possible assignment of the $n/k$ variables in that group. We represent assignment of variables with vectors of length $n/k$. For each assignment of variables $\vec{a}$ we create a vector $\vec{v}_{\vec{a}}$ of length $m$ where $\vec{v}_{\vec{a}}[j]$ is a $0$ if one of the variables in that clause is set true by the assignment $\vec{a}$ and is a $1$ otherwise. Note that the assignment $\vec{a}$ only sets $n/k$ of the variables. So, the clause can be fully unset, or have some variables set false and some variables unset and in these cases the clause is set to $1$. %If one variable is true we set the clause to zero regardless of the settings of the other variables. Finally we add $k$ more indices where index $m-1+\Delta$ is $0$ if this vector is produced by evaluation over $S_i$.
Now note that if we have one vector from each list such that there is at least one zero in each index between all $k$ vectors then the corresponding full assignment of variables satisfies the original formula $\oplus SAT$. There are $k2^{n/k}$ vectors $\vec{v}_{\vec{a}}$ and evaluating each index of the vector takes at most $O(n)$ time and there are $m$ indices in the vector. So building the $k$-OV instance takes $O(k2^{n/k}nm)$ time.

The resulting instance of $\oplus k$-OV has the same number of solutions as the $\oplus$SAT instance did. Every solution of the $\oplus k$-OV instance corresponds to exactly one satisfying assignment. Every satisfying assignment corresponds to exactly one $\oplus k$-OV witness. 
\end{proof}

Now we will apply this reduction to the SAT instances from Theorem \ref{thm:AvgCaseHardSAT}.
First let us define the distribution of $\oplus k$-OV instances.

\begin{definition}
Recall that the distribution $D_{\oplus SAT(b,g,\ell)}^N$ results from applying the reduction of Theorem \ref{thm:fkov-sat} to $\oplus $\ckov[\ell]$(N,b,g)$ with uniform input. 
Let $D^{N}_{\oplus OV(b,g,\ell,k)}$ be the distribution that results from applying the reduction of Lemma \ref{lem:SATtoOVWorstCase} to an instance of SAT drawn from $D^{N}_{\oplus SAT(b,g,\ell)}$.
\end{definition}

%Now we can explore the implications of reducing to $\oplus k$-OV. 


\begin{lemma}
Let $b=o(n)$ and $g=o(n)$ and $bg=m=\Theta(n)$. 
%Let $\hat{n}= n+\ell b g$ and let $\hat{m}=2^{n/\ell+b}g\ell+bg$. 
Let $\ell=\lg(\lg(\lg(n)))$, $k=\Theta(\ell)$, and $N=2^{n/\ell}$.
Any algorithm that solves instances of $\oplus k$-OV drawn from $D^{N}_{\oplus OV(b,g,\ell,k)}$  with probability $1-2^{-g\ell-3}$ requires $N^{\Omega{(k)}}$ time under rETH.

%where $N$ is the number of vectors in each of the $k$ lists and $D$ is the dimension of the vectors.
%If $T(N,D) = \poly(D)N^{o(k)}$ and $p>1-2^{-g\ell-2}$ then ErTH is false.
\label{lem:SATtoOVFirstPass}
\end{lemma}
\begin{proof}
Suppose rETH is true and an algorithm $\alg$ exists that solves instances of $\oplus k$-OV drawn from $D^{N}_{\oplus OV(b,g,\ell,k)}$  with probability $1-2^{-g\ell-3}$ in $N^{o(k)}$ time. 

We will first use Theorem \ref{thm:AvgCaseHardSAT}. Recall that it states: If an algorithm, $\alg$ exists for $\ell=\lg(\lg(\lg(n)))$ such that on an input $J$ drawn from $D^{N}_{\oplus SAT(b,g,\ell)}$,  $\alg$ returns the parity of the number of satisfying assignments to $J$ with probability $1-2^{-g\ell-3}$ in time $2^{o(n)}$ then rETH is false. 

We can now apply Lemma \ref{lem:SATtoOVWorstCase} in time $O(k2^{n/k})=2^{o(n)}$ to the instance $J$ to get an instance $I$ drawn from $D^{N}_{\oplus OV(b,g,\ell,k)}$ and run $\alg$ on $I$. This means that Lemma \ref{lem:SATtoOVWorstCase} and algorithm $\alg$ serve as an algorithm $\alg'$ on $\oplus$SAT with inputs drawn from $D^{N}_{\oplus SAT(b,g,\ell)}$, such that $\alg'$ has success probability $1-2^{g\ell -3}$ and runs in time $O(N^{o(k)})$ time. Note that $N=2^{n/\ell}$ and $k=O{(\ell)}$, so $N^{o(k)}=2^{o(n)}$, and hence by Theorem \ref{thm:AvgCaseHardSAT} this is a contradiction to rETH.
%Now an algorithm for solving $I$ in time $N^{o(k)}$ with probability $p$ would imply an algorithm for average-case $\oplus$SAT which runs in time $2^{n o(k)/k}$ with probability $p$. Now, if rETH is true then there is some constant $c$ such that solving $J \sim D^{2^{n/\ell}}_{\oplus SAT(b,g,\ell)}$ in time $poly(\hat{m}) \cdot 2^{n/c}$ for all $\ell$ is impossible (if no such $c$ exists then a solver running time $poly(\hat{m}) \cdot 2^{o(n)}$ would exist). So, if the algorithm $\alg$ ran in time $T(N,D) = \poly(D)N^{o(k)}$ we could, for any given $\ell$, set $k$ large enough that $o(k)/k<1/c$ for any given $c$. As a result, we would violate rETH by using Theorem \ref{thm:AvgCaseHardSAT} and Lemma \ref{lem:SATtoOVWorstCase}.
\end{proof}

We can now plug in values for $b$ and $g$ to get a cleaner statement. 


\sattoovhardness*
\begin{proof}
Let $g=\lg(\lg(n))/\ell$ and $b=n/g$. We only need to apply Lemma \ref{lem:SATtoOVFirstPass} with these values.
%We plug in $b=g=\Theta(\sqrt{n})$ to Lemma \ref{lem:SATtoOVFirstPass}. This gives our cleaner statement. 
\end{proof}

%Now we will note the relationship of $D$ and $N$ in these instances. We are starting with a SAT worst-case SAT instance with $n$ variables and $m=cn$ clauses for some fixed constant $c$. We apply the reductions of Section \ref{sec:avgCaseSat} as well as the reduction from Lemma \ref{lem:SATtoOVFirstPass}. First, we will note the number of vectors $N=2^{(n+\ell bg)/k} = 2^{(n+ \ell m)/k} = 2^{\ell c n/k}$. Now we will note the dimension is equal to $\hat{m}$, the number of clauses in the SAT instances produced for Theorem \ref{thm:AvgCaseHardSAT}. This means that $D= \hat{m} = 2^{n/\ell+b}g\ell+bg = 2^{n/\ell +o(n)}$. So, when $\ell$ and $k$ are arbitrarily large constants the relative size of $N$ and $D$ can be stated as $D =N^{k/(\ell^2 c)}$. Now we can consider the relative size of $k$ and $\ell$. We can choose $\ell$ to be arbitrarily large and $k=\ell^{1.5}$. Now as we grow $\ell$ the relative size of the vectors compared to the number of vectors shrinks: $D=N^{\Theta(\ell^{-0.5})}$. Additionally, as $\ell$ grows $N$ gets arbitrarily smaller than $2^n$. 





==> oldabstract.tex <==
This paper establishes conditional lower bounds for average-case {\em parity}-counting versions of the problems $k$-XOR, $k$-SUM, and $k$-OV. We demonstrate the following worst-case to average-case {\em self-reductions} for these problems: 
\begin{itemize}
    \item Assuming the $k$-OV hypothesis for randomized algorithms in the worst case, $\paritykOV$  is $n^{\Theta(\sqrt{k})}$ average-case hard.
    \item 
    Assuming the $k$-SUM hypothesis for randomized algorithms in the worst case,  $\paritykSUM$  is $n^{\Theta(\sqrt{k})}$  average-case hard.
    \item Assuming the $k$-XOR hypothesis for randomized algorithms  in the worst case,  $\paritykXOR$  is $n^{\Theta(\sqrt{k})}$  average case hard.
\end{itemize}
These results are the first to show that $\paritykOV$, $\paritykXOR$, and $\paritykSUM$ are hard under specific distributions derived from their worst-case versions. We additionally show $n^{\Theta(\sqrt{k})}$  average-case hardness for these problems from the $k$-clique hypothesis.

To achieve these results, we present a novel and improved framework for worst-case to average-case fine-grained reductions, building on the work of Dalirooyfard, Lincoln, and Vassilevska Williams (FOCS 2020).
